Neural Body: Implicit Neural Representations with Structured Latent Codes for Novel View Synthesis of Dynamic Humans

This paper addresses the challenge of novel view synthesis for a human performer from a very sparse set of camera views. Some recent works have shown that learning implicit neural representations of 3D scenes achieves remarkable view synthesis quality given dense input views. However, the representation learning will be ill-posed if the views are highly sparse. To solve this ill-posed problem, our key idea is to integrate observations over video frames. To this end, we propose Neural Body, a new human body representation which assumes that the learned neural representations at different frames share the same set of latent codes anchored to a deformable mesh, so that the observations across frames can be naturally integrated. The deformable mesh also provides geometric guidance for the network to learn 3D representations more efficiently. To evaluate our approach, we create a multi-view dataset named ZJU-MoCap that captures performers with complex motions. Experiments on ZJU-MoCap show that our approach outperforms prior works by a large margin in terms of novel view synthesis quality. We also demonstrate the capability of our approach to reconstruct a moving person from a monocular video on the People-Snapshot dataset. The code and dataset are available at https://zju3dv.github.io/neuralbody/.

==> table/02_multi_view_ssim_result.tex <==
\begin{table}
\tablestyle{4pt}{1.05}
\begin{tabular}{c|x{35}x{28}x{24}x{20}|x{28}x{20}}
& \multicolumn{4}{c|}{Frame 1} & \multicolumn{2}{c}{All video frames} \\[.1em]
\shline
& NeRF \cite{mildenhall2020nerf} & NV \cite{lombardi2019neural} & OURS* & OURS & NV \cite{lombardi2019neural} & OURS \\
\hline
Twirl  & 0.776 & 0.868 & 0.940 & \textbf{0.970} & 0.861 & \textbf{0.971} \\
Taichi & 0.681 & 0.748 & 0.806 & \textbf{0.950} & 0.824 & \textbf{0.962} \\
Swing1 & 0.729 & 0.694 & 0.883 & \textbf{0.939} & 0.726 & \textbf{0.946} \\
Swing2 & 0.743 & 0.833 & 0.881 & \textbf{0.940} & 0.843 & \textbf{0.940} \\
Swing3 & 0.832 & 0.880 & 0.921 & \textbf{0.949} & 0.842 & \textbf{0.939} \\
Warmup & 0.773 & 0.835 & 0.902 & \textbf{0.950} & 0.842 & \textbf{0.951} \\
Punch1 & 0.760 & 0.774 & 0.889 & \textbf{0.922} & 0.820 & \textbf{0.931} \\
Punch2 & 0.769 & 0.845 & 0.899 & \textbf{0.933} & 0.838 & \textbf{0.928} \\
Kick   & 0.769 & 0.817 & 0.897 & \textbf{0.925} & 0.825 & \textbf{0.926} \\
\hline                    
average & 0.759 & 0.810 & 0.891 & \textbf{0.942} & 0.825 & \textbf{0.944} \\
\end{tabular}
\caption{\textbf{Results on the ZJU-MoCap dataset in terms of SSIM (higher is better).} ``NV" means Neural Volumes, and ``OURS*" and ``OURS" represents our models trained only on the first video frame and all frames, respectively. We test these methods on ``Frame 1" and ``All video frames".}
\vspace{-3mm}
\label{table:multi_view_ssim}
\end{table}

